BlueFlood: Concurrent Transmissions for Multi-Hop Bluetooth 5 -- Modeling and Evaluation

Bluetooth is an omnipresent technology, available on billions of devices today. While it has been traditionally limited to peer-to-peer communication and star networks, the recent Bluetooth Mesh standard extends it to multi-hop networking. In addition, the Bluetooth 5 standard introduces new modes to allow for increased reliability. In this paper, we evaluate the feasibility of concurrent transmissions (CT) in Bluetooth via modeling and controlled experiments and then devise an efficient network-wide data dissemination protocol, BlueFlood, based on CT for multi-hop Bluetooth networks. First, we model and analyze how CT distorts the received waveform and characterize the Bit Error Rate of a Frequency-Shift Keying receiver to show that CT is feasible over Bluetooth. Second, we verify our analytic results with a controlled experimental study of CT over Bluetooth PHY. Third, we present BlueFlood, a fast and efficient network-wide data dissemination in multi-hop Bluetooth networks. In our experimental evaluation, in two testbeds deployed in university buildings, we show that BlueFlood achieves 99.9% end-to-end delivery ratio with a duty-cycle of 0.4% for periodic dissemination of advertising packets of 38 bytes with 200 milliseconds intervals at 2 Mbps. Moreover, we show that BlueFlood can be received by off-the-shelf devices such as smartphones, paving a seamless integration with existing technologies.

==> Makefile <==
DOC?=main
NAME?=blueflood_tiot
PACKAGE=acmart
#https://github.com/google-research/arxiv-latex-cleaner
ARXIV_CLEANER_PATH=/Users/beshr/work/arxiv-latex-cleaner/
RemoveACM?=0

.PHONY: pdf

.PHONY: preview

%.cls:   %.ins %.dtx
	pdflatex $<

#$(PACKAGE).cls ACM-Reference-Format.bst
pdf:
	pdflatex -file-line-error -interaction=nonstopmode $(DOC).tex
	bibtex $(DOC)
	pdflatex -file-line-error -interaction=nonstopmode $(DOC).tex
	pdflatex -file-line-error -interaction=nonstopmode $(DOC).tex
	bibtex $(DOC)
	pdflatex -file-line-error -interaction=nonstopmode $(DOC).tex
	pdflatex -file-line-error -interaction=nonstopmode --synctex=-1 $(DOC).tex
	while (grep -q '^LaTeX Warning: Label(s) may have changed' $(DOC).log) \
	do pdflatex -file-line-error -interaction=nonstopmode --synctex=-1 $(DOC).tex; done

pdfewsn: 
	pdflatex -file-line-error -interaction=nonstopmode $(DOC).tex
	bibtex $(DOC)
	pdflatex -file-line-error -interaction=nonstopmode $(DOC).tex
	pdflatex -file-line-error -interaction=nonstopmode --synctex=-1 $(DOC).tex
	while (grep -q '^LaTeX Warning: Label(s) may have changed' $(DOC).log) \
	do pdflatex -file-line-error -interaction=nonstopmode --synctex=-1 $(DOC).tex; done

pdfewsn2:
	/Library/TeX/texbin/pdflatex -file-line-error -halt-on-error $(DOC).tex
	/Library/TeX/texbin/bibtex $(DOC)
	/Library/TeX/texbin/pdflatex -file-line-error -halt-on-error $(DOC).tex
	/Library/TeX/texbin/pdflatex -file-line-error -halt-on-error --synctex=-1 $(DOC).tex
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(DOC).log) \
	do /Library/TeX/texbin/pdflatex -file-line-error --synctex=-1 $(DOC).tex; done
	gs -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -dEmbedAllFonts=true -dFirstPage=1 -dLastPage=12 -sOutputFile=$(DOC)2.pdf -f $(DOC).pdf
	#pdffonts $(DOC)
	#pdf2ps $(DOC)
	#ps2pdf14 -dPDFSETTINGS=/prepress $(DOC).ps $(DOC)2.pdf

plots-pdf:
	#if [ -f plots/*.pdf ]; then for f in plots/*.pdf; do echo "Cropping $$f"; pdfcrop $$f $$f; done fi
	#for f in plots/*.pdf; do if [[ -f plots/*.pdf ]]; then echo "Cropping $$f"; pdfcrop $$f $$f; fi; done
	for f in plots/*.pdf; do echo "Cropping $$f"; pdfcrop $$f $$f; done

gfx-pdf:
	#if [ -f plots/*.pdf ]; then for f in plots/*.pdf; do echo "Cropping $$f"; pdfcrop $$f $$f; done fi
	#for f in plots/*.pdf; do if [[ -f plots/*.pdf ]]; then echo "Cropping $$f"; pdfcrop $$f $$f; fi; done
	for f in gfx/*.pdf; do echo "Cropping $$f"; pdfcrop $$f $$f; done

pics-pdf:
	#for f in pics/*.pdf; do echo "Cropping $$f"; pdfcrop $$f $$f; done
	#for f in pics/*.pdf; do if [ -f pics/*.pdf ]; then echo "Cropping $$f"; pdfcrop $$f $$f; fi; done
	for f in pics/*.pdf; do echo "Cropping $$f"; pdfcrop $$f $$f; done

plots-png:
	for f in plots/*.pdf; do echo "Converting to PNG: $$f"; gs -dNOPAUSE -sDEVICE=png16m -r256 -sOutputFile=$$f.png $$f; done

test:
	for f in gfx/*.eps; do echo "Convert $${f} $${f%.eps}.pdf"; done;

eps2pdf:
	mkdir -p doNotUpload/gfxeps ;\
	if [[ $$(ls -1  gfx/*.eps  2>/dev/null | grep -c '^') != "0" ]]; then \
	for f in gfx/*.eps; do echo "Convert $$f"; ps2pdf $${f} $${f%.eps}.pdf; done; \
	mv gfx/*.eps doNotUpload/gfxeps/ ;\
	for f in gfx/*.pdf; do echo "Crop $$f"; pdfcrop $$f $$f; done; \
	fi;

prepareForArxiv:
	if [[ "$${RemoveACM}" == "1" ]]; then \
	sed "s=\(^\%\\\arxivMode$$\)=\\\arxivMode=" -i main.tex || true; \
	else \
	true || sed "s=\(^\\\arxivMode$$\)=\%\\\arxivMode=" -i main.tex || true ; \
	fi;
	sed "s=\(^\\\reviewMode$$\)=\%\\\reviewMode=" -i main.tex || true ;

removeExtraFiles:
	mkdir -p doNotUpload/pics ;\
	mkdir -p doNotUpload/plots ;\
	if [[ $$(ls -1 *.txt 2>/dev/null | grep -c '^') != "0" ]]; then mv *.txt doNotUpload/ ; fi;\
	if [[ $$(ls -1 *.docx 2>/dev/null | grep -c '^') != "0" ]]; then mv *.docx doNotUpload/ ; fi;\
	if [[ $$(ls -1  pics/*.png  2>/dev/null | grep -c '^') != "0" ]]; then mv pics/*.png doNotUpload/pics/ ; fi;\
	if [[ $$(ls -1  pics/*.pptx  2>/dev/null | grep -c '^') != "0" ]]; then mv pics/*.pptx doNotUpload/pics/ ; fi;\
	if [[ $$(ls -1  plots/*.png  2>/dev/null | grep -c '^') != "0" ]]; then mv plots/*.png doNotUpload/plots/ ; fi;\
	if [[ $$(ls -1  plots/*.pptx  2>/dev/null | grep -c '^') != "0" ]]; then mv plots/*.pptx doNotUpload/plots/ ; fi;\

prepareSubmission: prepareForArxiv removeExtraFiles
	WDIR=$$(pwd); echo $${WDIR} ;\
	rm -rf ../ble-tiot_arXiv/ ;\
	pushd ${ARXIV_CLEANER_PATH} ;\
	python -m arxiv_latex_cleaner $${WDIR}/ --commands_to_delete "\todo{} \ba{} \ol{} \sd{} \sketch{} \st{}" ;\
	popd;\
	cp $(DOC).bbl ../ble-tiot_arXiv/ ;\
	cp paper.bib ../ble-tiot_arXiv/ ;\
	cp Makefile ../ble-tiot_arXiv/ ; pushd ../ble-tiot_arXiv/ ; make pdf ; cp $(DOC).pdf /tmp/ ; make clean; rm -rf $(DOC).synctex; zip -9 -r $(NAME)_arxiv_submission.zip . -x .* ; popd; mv ../ble-tiot_arXiv/$(NAME)_arxiv_submission.zip ./ ; cp /tmp/$(DOC).pdf $(NAME)_arxiv.pdf ; open -a Preview $(NAME)_arxiv.pdf ;

prepareSubmissionACM: prepareForArxiv removeExtraFiles
	WDIR=$$(pwd); echo $${WDIR} ;\
	rm -rf ../ble-tiot_arXiv/ ;\
	pushd ${ARXIV_CLEANER_PATH} ;\
	python -m arxiv_latex_cleaner $${WDIR}/ --commands_to_delete "\todo{} \ba{} \ol{} \sd{} \sketch{} \st{}" ;\
	popd;\
	cp $(DOC).bbl ../ble-tiot_arXiv/ ;\
	cp paper.bib ../ble-tiot_arXiv/ ;\
	cp Makefile ../ble-tiot_arXiv/ ; pushd ../ble-tiot_arXiv/ ; make pdf ; cp $(DOC).pdf /tmp/ ; make clean; rm -rf $(DOC).synctex; zip -9 -r $(NAME)_acm_submission.zip . -x .* ; popd; mv ../ble-tiot_arXiv/$(NAME)_acm_submission.zip ./ ; cp /tmp/$(DOC).pdf $(NAME)_acm.pdf ; open -a Preview $(NAME)_acm.pdf ;

preview:
	open -a Preview $(DOC).pdf 

all: plots-pdf pics-pdf pdfewsn

clean:
	rm -f $(DOC).blg $(DOC).aux $(DOC).log $(DOC).pdf *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

